Interpolative Decomposition Butterfly Factorization

This paper introduces a "kernel-independent" interpolative decomposition butterfly factorization (IDBF) as a data-sparse approximation for matrices that satisfy a complementary low-rank property. The IDBF can be constructed in $O(N\log N)$ operations for an $N\times N$ matrix via hierarchical interpolative decompositions (IDs), if matrix entries can be sampled individually and each sample takes $O(1)$ operations. The resulting factorization is a product of $O(\log N)$ sparse matrices, each with $O(N)$ non-zero entries. Hence, it can be applied to a vector rapidly in $O(N\log N)$ operations. IDBF is a general framework for nearly optimal fast matvec useful in a wide range of applications, e.g., special function transformation, Fourier integral operators, high-frequency wave computation. Numerical results are provided to demonstrate the effectiveness of the butterfly factorization and its construction algorithms.

==> figure/fig-IDex.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{1.5cm}{!}{
\input{figure/fig-comp-modules/fig-id-A1}
}
$\approx$
\resizebox{1.5cm}{!}{
\input{figure/fig-comp-modules/fig-id-A1u}
}
\resizebox{1.5cm}{!}{
\input{figure/fig-comp-modules/fig-id-A1s}
} 
\ \ \ \ \ \  
\resizebox{1.5cm}{!}{
\input{figure/fig-comp-modules/fig-id-A2}
}
$\approx$
\resizebox{1.5cm}{!}{
\input{figure/fig-comp-modules/fig-id-A2s}
}
\resizebox{1.5cm}{!}{
\input{figure/fig-comp-modules/fig-id-A2v}
}\\ 
\end{minipage}
\caption{The left is a (row) ID of a short fat matrix, the right is a (column) ID of a tall skinny matrix. }
\label{fig:IDex}
\end{figure}

==> figure/fig-chpart-ex.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{1.0cm}{!}{
\input{figure/fig-comp-modules/fig-chpart-o}
}
\quad
\resizebox{1.0cm}{!}{
\input{figure/fig-comp-modules/fig-chpart-or}
}
\quad
\resizebox{1.0cm}{!}{
\input{figure/fig-comp-modules/fig-chpart-oc}
}
\quad previous-level blocking \   
\\
\resizebox{0.95cm}{!}{
}\quad \quad \quad
\resizebox{1.0cm}{!}{
\input{figure/fig-comp-modules/fig-chpart-cr}
}
\quad
\resizebox{1.0cm}{!}{
\input{figure/fig-comp-modules/fig-chpart-cc}
}
\quad double-and-halve blocking

\end{minipage}
\caption{An illustration of changing partition. The top-left matrix represents one of blocks in  $S^{4}$ in (\ref{eq:expressUSV4}) or Figure \ref{fig:exlfac}, the top-middle and top-right ones visualize the previous-level partition of rows and columns of the block, respectively. The bottom-left and bottom-right ones visualize the double-and-halve process on the block for next level, as shown in (\ref{eq:exdoubleins}) and (\ref{eq:exS4next}).  }
\label{fig:chpart}
\end{figure}

==> figure/fig-comp-modules/fig-chpart-o.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
      \draw;
\draw[fill=gray] (0,0) rectangle (8,8);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-u1.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,2,...,30}{
\foreach \i in {0,0.5,...,1.5} {
    \draw[fill=gray] (32-\i-\k,\k) rectangle (32-\i-\k-0.5,\k+2);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-u2.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,1,...,31}{
\foreach \i in {0,0.5} {
    \draw[fill=gray] (32-\i-\k,\k) rectangle (32-\i-\k-0.5,\k+1);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-v1.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,2,...,30}{
\foreach \i in {0,0.5,...,1.5} {
    \draw[fill=gray] (\k,32-\i-\k) rectangle (\k+2,32-\i-\k-0.5);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-comp-v2.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,1,...,31}{
\foreach \i in {0,0.5} {
    \draw[fill=gray] (\k,32-\i-\k) rectangle (\k+1,32-\i-\k-0.5);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-id-A1.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw[fill=gray] (0,0) rectangle (16,8);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-id-A1U.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw[fill=gray] (0,0) rectangle (4,8);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-id-A1s.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw[fill=gray] (0,0) rectangle (16,4);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-id-A2.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw[fill=gray] (0,0) rectangle (8,16);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-id-A2s.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw[fill=gray] (0,0) rectangle (4,16);
\\
      };
\end{tikzpicture}

==> figure/fig-comp-modules/fig-id-A2v.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw[fill=gray] (0,0) rectangle (8,4);
\\
      };
\end{tikzpicture}

==> figure/fig-compression-1D.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-K}
}
$\approx$
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-u}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-M}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-v}
}\\
\end{minipage}
\caption{The middle level factorization of
    a $64\times 64$ complementary low-rank matrix $K\approx U^3M^3(V^3)^*$
    assuming $r=1$.
    Grey blocks indicate nonzero blocks.
    $U^3$ and $V^3$ are block-diagonal matrices with $8$ blocks.
    The diagonal blocks of $U^3$ and $V^3$ are assembled
    according to Equation \eqref{eq:expression-UV}
    as indicated by black rectangles.
    $M^3$ is a $8\times 8$ block matrix with each block
    $M^3_{i,j}$ itself an $8\times 8$ block matrix
    containing diagonal weights matrix on the $(j,i)$ block.}
\label{fig:compression-1D}
\end{figure}


==> figure/fig-compression-1D2.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-u2}
}
$\approx$
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-svd}
}
=
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-u1}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-g1}
}\\
\resizebox{3.5cm}{!}{
}
$\approx$
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-u2}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-g2}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-g1}
}\\
\end{minipage}
\caption{The recursive factorization of $U^3$
    in Figure~\ref{fig:compression-1D}.
    Gray factors are matrices inheriting the complementary low-rank
    property.
    Top: left matrix: $U^3$ with each diagonal block
    partitioned into smaller blocks according to
    Equation \eqref{eqn:half} as indicated by black rectangles;
    middle-left matrix: low-rank approximations of submatrices
    in $U^3$ given by Equation \eqref{eqn:RSh};
    middle right matrix: $U^4$;
    right matrix: $G^3$.
    Bottom: $U^4$ in the first row is further factorized into
    $U^4\approx U^5G^4$, giving $U^3 \approx U^5 G^4 G^3$.}
\label{fig:compression-1D2}
\end{figure}

==> figure/fig-compression-1D3.tex <==
\begin{figure}[htp]
\begin{minipage}{\textwidth}
\centering
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-uncomp-v2}
}
=
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-h1}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-h2}
}
\resizebox{3.5cm}{!}{
\input{figure/fig-comp-modules/fig-comp-v2}
}\\
\end{minipage}
\caption{The recursive factorization $(V^3)^* \approx (H^3)^*(H^4)^*(V^5)^*$ of $(V^3)^*$
    in Figure~\ref{fig:compression-1D}.}
\label{fig:compression-1D3}
\end{figure}


==> figure/fig-domain-tree-1D.tex <==
\begin{figure}[htp]
\centering
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}[scale=0.4]

\draw [->,double,double distance=1pt] (2,-1.2) -> (2,-2.8);

\draw [|-|] (0,0) -- (2,0);
\draw [|-|] (2,0) -- (4,0);

\draw [|-|] (0,-4) -- (1,-4);
\draw [|-|] (1,-4) -- (2,-4);
\draw [|-|] (2,-4) -- (3,-4);
\draw [|-|] (3,-4) -- (4,-4);

\draw [->,double,double distance=1pt] (2+12,1.2) -> (2+12,2.8);

\draw [|-|] (0+12,4) -- (4+12,4);

\draw [|-|] (0+12,0) -- (2+12,0);
\draw [|-|] (2+12,0) -- (4+12,0);

\draw [latex-latex,line width=1pt] (10,4) -> (6,-4);
\draw [latex-latex,line width=1pt] (10,0) -> (6,0);

\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}[scale=0.4]

\draw [->,double,double distance=1pt] (2,1.2) -> (2,2.8);

\draw [|-|] (0,4) -- (4,4);

\draw [|-|] (0,0) -- (2,0);
\draw [|-|] (2,0) -- (4,0);


\draw [->,double,double distance=1pt] (2+12,-1.2) -> (2+12,-2.8);

\draw [|-|] (0+12,0) -- (2+12,0);
\draw [|-|] (2+12,0) -- (4+12,0);

\draw [|-|] (0+12,-4) -- (1+12,-4);
\draw [|-|] (1+12,-4) -- (2+12,-4);
\draw [|-|] (2+12,-4) -- (3+12,-4);
\draw [|-|] (3+12,-4) -- (4+12,-4);

\draw [latex-latex,line width=1pt] (10,0) -> (6,0);
\draw [latex-latex,line width=1pt] (10,-4) -> (6,4);

\end{tikzpicture}
\end{minipage}
\caption{1D {FIO} domain tree. The left figure shows the compression of $U$
    and the right figure shows the compression of $V$.
    In each figure, the left column shows target subdomains
    and the right column shows source subdomains;
    the solid double-head arrows show the low-rank interactions;
    the double line arrow shows the direction for the splitting and merging of subdomains. }
\label{fig:domain-tree-1D}
\end{figure}


==> figure/fig-domain-tree-2D.tex <==
\begin{figure}[htp]
\centering
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}[scale=0.4]

\draw [->,double,double distance=1pt] (2,-1.2,2) -> (2,-2.8,2);

\draw (0,0,0) -- (0,0,2) -- (2,0,2) -- (2,0,0) -- cycle;
\draw (0,-4,0) -- (0,-4,1) -- (1,-4,1) -- (1,-4,0) -- cycle;
\draw (1,-4,1) -- (1,-4,2) -- (2,-4,2) -- (2,-4,1) -- cycle;
\draw (1,-4,0) -- (1,-4,1) -- (2,-4,1) -- (2,-4,0) -- cycle;
\draw (0,-4,1) -- (0,-4,2) -- (1,-4,2) -- (1,-4,1) -- cycle;

\draw (2,0,0) -- (2,0,2) -- (4,0,2) -- (4,0,0) -- cycle;
\draw (2,-4,0) -- (2,-4,1) -- (3,-4,1) -- (3,-4,0) -- cycle;
\draw (3,-4,1) -- (3,-4,2) -- (4,-4,2) -- (4,-4,1) -- cycle;
\draw (3,-4,0) -- (3,-4,1) -- (4,-4,1) -- (4,-4,0) -- cycle;
\draw (2,-4,1) -- (2,-4,2) -- (3,-4,2) -- (3,-4,1) -- cycle;

\draw (2,0,2) -- (2,0,4) -- (4,0,4) -- (4,0,2) -- cycle;
\draw (2,-4,2) -- (2,-4,3) -- (3,-4,3) -- (3,-4,2) -- cycle;
\draw (3,-4,3) -- (3,-4,4) -- (4,-4,4) -- (4,-4,3) -- cycle;
\draw (3,-4,2) -- (3,-4,3) -- (4,-4,3) -- (4,-4,2) -- cycle;
\draw (2,-4,3) -- (2,-4,4) -- (3,-4,4) -- (3,-4,3) -- cycle;

\draw (0,0,2) -- (0,0,4) -- (2,0,4) -- (2,0,2) -- cycle;
\draw (0,-4,2) -- (0,-4,3) -- (1,-4,3) -- (1,-4,2) -- cycle;
\draw (1,-4,3) -- (1,-4,4) -- (2,-4,4) -- (2,-4,3) -- cycle;
\draw (1,-4,2) -- (1,-4,3) -- (2,-4,3) -- (2,-4,2) -- cycle;
\draw (0,-4,3) -- (0,-4,4) -- (1,-4,4) -- (1,-4,3) -- cycle;

\draw [->,double,double distance=1pt] (2+12,1.2,2) -> (2+12,2.8,2);

\draw (0+12,4,0) -- (0+12,4,4) -- (4+12,4,4) -- (4+12,4,0) -- cycle;

\draw (0+12,0,0) -- (0+12,0,2) -- (2+12,0,2) -- (2+12,0,0) -- cycle;
\draw (2+12,0,0) -- (2+12,0,2) -- (4+12,0,2) -- (4+12,0,0) -- cycle;
\draw (2+12,0,2) -- (2+12,0,4) -- (4+12,0,4) -- (4+12,0,2) -- cycle;
\draw (0+12,0,2) -- (0+12,0,4) -- (2+12,0,4) -- (2+12,0,2) -- cycle;

\draw [latex-latex,line width=1pt] (10,0,2) -> (6,0,2);
\draw [latex-latex,line width=1pt] (10,4,2) -> (6,-4,2);

\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}[scale=0.4]

\draw [->,double,double distance=1pt] (2,1.2,2) -> (2,2.8,2);

\draw (0,4,0) -- (0,4,4) -- (4,4,4) -- (4,4,0) -- cycle;

\draw (0,0,0) -- (0,0,2) -- (2,0,2) -- (2,0,0) -- cycle;
\draw (2,0,0) -- (2,0,2) -- (4,0,2) -- (4,0,0) -- cycle;
\draw (2,0,2) -- (2,0,4) -- (4,0,4) -- (4,0,2) -- cycle;
\draw (0,0,2) -- (0,0,4) -- (2,0,4) -- (2,0,2) -- cycle;

\draw [->,double,double distance=1pt] (2+12,-1.2,2) -> (2+12,-2.8,2);

\draw (0+12,0,0) -- (0+12,0,2) -- (2+12,0,2) -- (2+12,0,0) -- cycle;
\draw (0+12,-4,0) -- (0+12,-4,1) -- (1+12,-4,1) -- (1+12,-4,0) -- cycle;
\draw (1+12,-4,1) -- (1+12,-4,2) -- (2+12,-4,2) -- (2+12,-4,1) -- cycle;
\draw (1+12,-4,0) -- (1+12,-4,1) -- (2+12,-4,1) -- (2+12,-4,0) -- cycle;
\draw (0+12,-4,1) -- (0+12,-4,2) -- (1+12,-4,2) -- (1+12,-4,1) -- cycle;

\draw (2+12,0,0) -- (2+12,0,2) -- (4+12,0,2) -- (4+12,0,0) -- cycle;
\draw (2+12,-4,0) -- (2+12,-4,1) -- (3+12,-4,1) -- (3+12,-4,0) -- cycle;
\draw (3+12,-4,1) -- (3+12,-4,2) -- (4+12,-4,2) -- (4+12,-4,1) -- cycle;
\draw (3+12,-4,0) -- (3+12,-4,1) -- (4+12,-4,1) -- (4+12,-4,0) -- cycle;
\draw (2+12,-4,1) -- (2+12,-4,2) -- (3+12,-4,2) -- (3+12,-4,1) -- cycle;

\draw (2+12,0,2) -- (2+12,0,4) -- (4+12,0,4) -- (4+12,0,2) -- cycle;
\draw (2+12,-4,2) -- (2+12,-4,3) -- (3+12,-4,3) -- (3+12,-4,2) -- cycle;
\draw (3+12,-4,3) -- (3+12,-4,4) -- (4+12,-4,4) -- (4+12,-4,3) -- cycle;
\draw (3+12,-4,2) -- (3+12,-4,3) -- (4+12,-4,3) -- (4+12,-4,2) -- cycle;
\draw (2+12,-4,3) -- (2+12,-4,4) -- (3+12,-4,4) -- (3+12,-4,3) -- cycle;

\draw (0+12,0,2) -- (0+12,0,4) -- (2+12,0,4) -- (2+12,0,2) -- cycle;
\draw (0+12,-4,2) -- (0+12,-4,3) -- (1+12,-4,3) -- (1+12,-4,2) -- cycle;
\draw (1+12,-4,3) -- (1+12,-4,4) -- (2+12,-4,4) -- (2+12,-4,3) -- cycle;
\draw (1+12,-4,2) -- (1+12,-4,3) -- (2+12,-4,3) -- (2+12,-4,2) -- cycle;
\draw (0+12,-4,3) -- (0+12,-4,4) -- (1+12,-4,4) -- (1+12,-4,3) -- cycle;

\draw [latex-latex,line width=1pt] (10,0,2) -> (6,0,2);
\draw [latex-latex,line width=1pt] (10,-4,2) -> (6,4,2);

\end{tikzpicture}
\end{minipage}
\caption{2D {FIO} domain tree. Left: splitting and merging directions for the factorization of the left factor in each factorization step. Right: splitting and merging directions for the factorization of the right factor in each factorization step.}
\label{fig:domain-tree-2D}
\end{figure}

==> figure/fig-domain-tree-BF.tex <==
\begin{figure}
\centering
\begin{tikzpicture}[scale=0.3]

\draw [->,double,double distance=1pt] (-6,9) -> (-6,1);

\draw (0,10) -- (-4,0) -- (4,0) -- cycle;

\draw [->,double,double distance=1pt] (20,1) -> (20,9);

\draw (14,10) -- (10,0) -- (18,0) -- cycle;

\draw [latex-latex,line width=1pt] (9,5) -> (5,5);
\draw [latex-latex,line width=1pt] (9,9) -> (5,1);
\draw [latex-latex,line width=1pt] (9,1) -> (5,9);

\coordinate [label=above:$T_X$] (X) at (0,10);
\coordinate [label=above:$T_\Omega$] (X) at (14,10);

\draw (-2,5) -- (2,5);
\draw (12,5) -- (16,5);

\coordinate [label=right:$\frac{L}{2}$] (X) at (16,5);
\coordinate [label=left:$\frac{L}{2}$] (X) at (-2,5);
\end{tikzpicture}
\caption{Trees of the row and column indices.
    Left: $T_X$ for the row indices $X$.
    Right: $T_\Omega$ for the column indices $\Omega$.
    The interaction between $A\in T_X$ and $B\in T_\Omega$
    starts at the root of $T_X$ and the leaves of $T_\Omega$. }
\label{fig:domain-tree-BF}
\end{figure}


==> figure/fig-double-block-matrix.tex <==
\begin{figure}[htp]
\begin{minipage}{0.32\textwidth}
\begin{tikzpicture}[scale=0.25]
\draw[draw=black] (0,0) rectangle (16,16);
\draw[draw=black,dashed] (0,8) rectangle (16,12);
\draw[draw=black,dashed] (8,0) rectangle (12,16);
\draw[draw=black] (8,8) rectangle (12,12);
\draw[draw=black,dashed] (9,8) rectangle (10,12);
\draw[draw=black,dashed] (8,9) rectangle (12,10);
\filldraw[fill=lightgray,draw=black] (9,9) rectangle (10,10);
\draw (0,10) node[left=3pt,rectangle,fill=white] {$A$};
\draw (10,16) node[above=3pt,rectangle,fill=white] {$B$};
\draw (8,9.5) node[left=3pt,rectangle,fill=white] {{\tiny $C$}};
\draw (9.5,12) node[above=3pt,rectangle,fill=white] {{\tiny $D$}};
\draw (8,0) node[below=5pt,rectangle,fill=white] {$M_{AB,CD}$};
\end{tikzpicture}
\end{minipage}
\caption{The visualization of the submatrices $\{M_{AB,CD}\}$, $\{M_{AB,:D}\}$, and $\{M_{AB,C:}\}$ in $M_{AB}$. The largest black rectangle represents a matrix $M$ and the smaller one inside $M$ indicates its submatrix $M_{AB}$. From left to right, the light gray boxes inside $M_{AB}$ indicate the submatrices  $\{M_{AB,CD}\}$, $\{M_{AB,:D}\}$, and $\{M_{AB,C:}\}$, respectively.}
\label{fig:double-block-matrix}
\end{figure}
